Temporally-Weighted Hierarchical Clustering for Unsupervised Action Segmentation

Action segmentation refers to inferring boundaries of semantically consistent visual concepts in videos and is an important requirement for many video understanding tasks. For this and other video understanding tasks, supervised approaches have achieved encouraging performance but require a high volume of detailed frame-level annotations. We present a fully automatic and unsupervised approach for segmenting actions in a video that does not require any training. Our proposal is an effective temporally-weighted hierarchical clustering algorithm that can group semantically consistent frames of the video. Our main finding is that representing a video with a 1-nearest neighbor graph by taking into account the time progression is sufficient to form semantically and temporally consistent clusters of frames where each cluster may represent some action in the video. Additionally, we establish strong unsupervised baselines for action segmentation and show significant performance improvements over published unsupervised methods on five challenging action segmentation datasets. Our code is available at https://github.com/ssarfraz/FINCH-Clustering/tree/master/TW-FINCH

==> tex_files/exp_old.tex <==
\iffalse
\textbf{Version 1-Testing:}

\textbf{Run-v1:} All results computed with following parameters, with hugarian matching. \textbf{accuracy: MoF} averaged over each video mof 

\textbf{Parameters:}

distance-weight-time-stamp = 50

\textbf{Null reference hypothesis params:}

B=20

alpha-sk= 2.5
\fi

\newpage

\section{Experiments}
In this section, we first introduce the datasets, metrics implementation details of our proposed approach.  Finally, we compare our unsupervised temporal segmentation method with baseline methods and other  state-of-the-art methods. Note that, the purpose of this paper is to improve the baseline segmentation performance via time-weighted clustering using generic hand-engineered IDT features, and not to compete against the trainable state-of-the-art methods.

\paragraph{\textbf{Datasets}} We conduct experiments on five challenging and popular temporal action segmentation datasets, namely the Breakfast dataset~(BF)~\cite{ute_15}, Inria Instructional Videos~(YTI)~\cite{yti_paper}, 50Salads~(FS)~\cite{fs_paper}, MPII Cooking 2~(MPII)~\cite{mpii_paper}, and Hollywood Extended~(HE)~\cite{he_paper}. Table~\ref{table:datasets} summarizes the statistics of each of these datasets. The number of videos~(\#Videos) in the different dataset varies from  50 to 1712, with average number of frames-per-video varies between 520 to 10555. The dimensionality of the data is 64 dimensions for all datasets except YTI  which is 3,000 dimensional. The datasets are challenging which cover different complex activities, such as Breakfast dataset has video of 10 kitchen preparation activities with an average 6 actions per video;  Inria Instructional Videos has narrated YouTube videos of 5 complex activities with an average of 9 action per video; 50Salads has videos of a single mixed salad making activity with an average of 19 actions per video;  MPII Cooking 2 has videos of 65 fine grained cooking activities with an average of 17 actions per video; and Hollywood Extended has videos of  16 different activies from  Hollywood movies with an average of 3 actions per video. The percentage of background frames varies between 7\% to 63.5\% frames of all frames in the dataset.

\begin{table}[t!]
%\tabcolsep=0.5cm
%\footnotesize
\centering
\resizebox{8.5cm}{!}{
\begin{tabular}{l|ccccc}
\toprule
& BF~\cite{ute_paper}    &   YTI~\cite{yti_paper} &   FS~\cite{fs_paper} &MPII~\cite{mpii_paper}  & HE~\cite{he_paper} \\
\midrule
\#Videos    & 1712  &   150 &   50 & 273    & 937 \\
%\# Avg. Frames per video    & 3.6M  & $\sim$450k & $\sim$500k     & 2.8M   & 800k    \\  
\# Avg. Frames-per-video     & 2099  & 520 &  11788     & 10555   & 835    \\  
Feature Dim.        & 64    &   3000&   64  &64      & 64  \\
\#Activities~(V)  & 10    &   5    &   1   & 67       & 16 \\  
Avg. \#Actions-per-video~(A)  & 6   &  9    &  19    &    17    & 3 \\  
%\#Actions/video~(A)  & 2 - 12    &  3-13    &  13-19    &    3-37    & 2-7 \\  
Background  & 7\% & 63.5\%  & 14.1\% & 29\% & 61\%\\
\bottomrule
\end{tabular}}
% \vspace{0.25cm}
\caption{Datasets used in the experiments. \textbf{A} denotes number of sub action classes known, V denotes the number video activity, A is the average number of actions-per-video and  Background refers to the \% of number of background frames in the whole dataset.\label{table:datasets}}
\end{table}


\paragraph{\textbf{Features}} For a fair comparison, we used the same features that were used by the recent methods~\cite{ute_paper,mallow,sct,cdfl,actionset} as their input.
For all datasets, feature-wise, we use  pre-computed reduced Fisher vectors available from UTE~\cite{ute_paper} (BF, YTI, FS) and SCT~\cite{sct} (MPII, HE).   The features are improved dense trajectories~\cite{idt} represented by PCA-projected to 64 dimension except YTI. For YTI~\cite{yti_paper}, the authors provide 3,000 dimensional feature vectors, concatenation of 2,000 dimensions HOF~\cite{hof} descriptors aggregated into a single bag-of-visual-word vector and 1,000 dimensions VGG16-conv5~\cite{vgg} activations aggregated into a single bag-of-visual-word vector. For all datasets, we report performance for the full dataset. %We also report performance for the test splits provided as the original evaluation scheme for these datasets.


\paragraph{\textbf{Metrics}} To evaluate the temporal segmentation, we need  one-to-one mappings between the predicted segment and ground-truth labels.  Following~\cite{ute_paper,mallow,cdfl,sct,actionset}, we use the Hungarian algorithm to get a one-to-one matching and then evaluate with four metrics: Accuracy as the mean over frames~(MoF); F1-score;  Jaccard index as the intersection over union~(IoU), midpoint hit criterion~\cite{rohrbach2012database} i.e. the midpoint of the predicted segment has to be within the groundtruth. We report MoF and IoU for all datasets, and in particular F1-score for YTI and midpoint hit for MPII as used in the previous works. For all metrics, a higher result indicates better performance.


\paragraph{\textbf{Evaluation Setup:}} Here, we describe the evaluation setup of our method, \textbf{TW1CH in unsupervised settings}.  In order to have a fair comparison to the recent methods~\cite{ute_paper,mallow,yti_paper,cdfl,sct,actionset} that all require a known number $K$ of actions in the videos, we also set $K$ based on the ground-truth.

%\textbf{$-$ TW1CH in fully unsupervised settings:} In this setup the number of ground-truth sub-activities are not known. In this case, we automatically estimate the number of sub-activities in the video.




\subsection{Comparison with the Baselines} To demonstrate the effectiveness of our TW1CH in unsupervised settings, in this section, we compare to the  baseline clustering methods that require a known number of $K$ ground-truth clusters; and  to the uniform splitting the number of frames in the video into $K$ parts (Equal Split).

Firstly, we compare our method to popular clustering methods: Kmeans~\cite{kmeans} and FINCH~\cite{finch}. For this comparison, we simply cluster the data with ground-truth $K$ clusters and then use Hungarian algorithm to perform one-to-one mapping between the predicted segments and the ground-truth segments. We can clearly observe that our method TW1CH (with given $K$) outperforms Kmeans and FINCH by a significant margin  on all five datasets, shown in Table~\ref{table:eval_bf}~(BF), Table~\ref{table:eval_yti}~(YTI), Table~\ref{table:eval_fs}~(FS), Table~\ref{table:eval_mpii}~(MPII) and Table~\ref{table:eval_he}~(HE). As previously discussed in Section~\ref{sec:method}, we establish a proper and strong baselines for the problem of temporal video segmentation and suggest that focusing on more specialized clustering techniques should perhaps be preferred. As one can easily observe that a simple baseline clustering using Kmeans or FINCH already provide quite a matching/better performance that the weakly supervised~\cite{cdfl,actionset,sct} and unsupervised methods~\cite{ute_paper,mallow,yti_paper}.

Second, we establish a strong \textit{Equal Split} baseline for temporal video segmentation where we perform uniform splitting the number of frames in the video into $K$ parts. Surprisingly, it is astonishing to see that in \textit{Equal Split} outperforms  weakly supervised,  baseline clustering, and unsupervised methods, in FS dataset~(Table~\ref{table:eval_fs}). A similar pattern could also be observed in BF dataset~(Table~\ref{table:eval_bf}), which complements our observation  that focusing on more specialized clustering techniques should be preferred as training the features drops the performance even below than Equal Split performance. TW1CH outperforms  Equal Split by a significant margin, indicating more semantically-meaningful right ordered clusters.


%As previously discussed in Section~\ref{sec:method}, as can be seen in direct comparison to the current best published unsupervised and weakly-supervised methods a simple clustering already provide quite a matching/better performance. This establishes a proper and strong baseline for the problem of temporal video segmentation and suggest that focusing on more specialized clustering techniques should perhaps be preferred.

%Surprisingly, it is interesting to see that in most of the case just baseline clustering using Kmeans or FINCH outperforms weakly supervised~\cite{cdfl,actionset,sct}  and unsupervised methods~\cite{ute_paper,mallow,yti_paper}.\naila{refer to similar discussion in method section. Must be rewritten if we are always using the number of classes $K$.}

%Furthermore, it is also interesting to observe that even with TW1CH automatically estimated segments, TW1CH still outperforms Kmeans and FINCH.

\subsection{Comparison with the State-of-the-art} We compare our proposed fully unsupervised method
%s: (1) TW1CH in unsupervised settings and (2) TW1CH in fully unsupervised settings
to current state-of-the-art unsupervised, weakly-supervised and fully-supervised approaches. We compare our method on five benchmark datasets: BF, YTI, FS, MPII, and HE. Note that we each dataset we report the standard metrics as proposed by the previous works, we also report IoU and MoF for future comparisons.  
%TW1CH performs the best among all methods in both setups and achieves state-of-the-art results on all five datasets, shown in Table~\ref{table:eval_bf}~(BF), Table~\ref{table:eval_yti}~(YTI), Table~\ref{table:eval_fs}~(FS), Table~\ref{table:eval_mpii}~(MPII) and Table~\ref{table:eval_he}~(HE).  
\saquib{I think a better way would be to have a small discussion on each dataset results separately, starting with few lines on the complexity of datasets and then mentioning our improvements related to the compared methods there}




\paragraph{Breakfast dataset~(BF):}\emph{ }

\textbf{Dataset.} The dataset contains an average of 6 actions per video, and 7\% of background frames of all frames in the whole dataset.   
% 6, 7%

\textbf{Results.} In Table~\ref{table:eval_bf}, we compare the performance of TW1CH with the current state-of-the-art unsupervised, weakly-supervised and fully-supervised approaches.  TW1CH performs the best among all methods.  TW1CH obtains an IoU of 44.1\% and MoF of 63.8\%.  TW1CH is -/22\%, 10.4/13.6\%, and -/2.5\% better than the UTE~\cite{ute_paper}, CDFL~\cite{cdfl}, RNN+HMM~\cite{kuehne2018hybrid} in IoU/MoF metric. Note that, our method outperforms the supervised method too.
%Further, TW1CH outperforms UTE~\cite{ute_paper} (in setup when the number of ground-truth action-categories are not known) by 45.5\% (63.8 $\rightarrow$  18.3) in MoF.

As previously discussed in Section~\ref{sec:method}, note that, our method only uses Hungarian algorithm for matching and still outperforms (1) UTE~\cite{ute_paper} that uses Viterbi decoding with Hungarian algorithm and (2) Mallow~\cite{mallow} that uses Generalized Mallows Model with Hungarian algorithm too. \naila{refer to similar discussion in method section}.

\textbf{Qualitative Results.}  In order to get a better understanding of our time-weighted clustering, in Fig.~\ref{fig:qual_ac} we show qualitative segmentation results on BF dataset. It is also interesting to observe that our method yields near perfect \textit{action} segmentation boundaries in most of the cases. 


\paragraph{Inria Instructional Videos~(YTI):}\emph{ }

\textbf{Dataset.} The dataset contains an average of 9 actions per video, and 63.5\% of background frames of all frames in the whole dataset. 
% 9 63.5\%

\textbf{Results.} In Table~\ref{table:eval_yti}, we summarize the performance of TW1CH and compare  it to state-of-the-art unsupervised, weakly-supervised and fully-supervised approaches. Note that for fair comparison with previous methods, for this evaluation we remove 75\% frames of all frames from the video sequence.Similar to BF dataset, TW1CH  outperforms other methods, and achieves F1-Score of 51.9/\% and MoF of 58.6\%, which is 23.6/19.6\%, 24.9/30.8\% and 27.5/-\% better than UTE~\cite{ute_paper}, Mallow~\cite{mallow} and Frank-Wolfe~\cite{yti_paper} in F1-Score/MoF metric. 

Next we compare our method to UTE by varying the number of background frame as direct comparison and show a simple clustering provide significant performance case.

\textbf{Impact of Background Frames.}  As actions in the videos are not necessarily executed in continuous temporal order, and rather has interruptions in between the actions, those frames that are not part of any action class are considered part of the background class.  As previously mentioned in Table~\ref{table:datasets}, almost every dataset has background frames varying between 7\% to 63.5\% frames of all frames in the whole dataset. The parameter $\tau$ defines the percentage of frames that are to be incorporated in the modeling.  Inria Instructional Videos~(YTI) dataset has been consider as a test bed by~\cite{ute_paper,mallow} to analyse the role background frame plays because 63.5\% frames in the whole dataset are background frames. Following the same setup as UTE~\cite{ute_paper}, to this end, we evaluate our TW1CH without background by removing $\tau$\% frames from the video sequence~(wo bg.) and with background by keeping $\tau$\% frames~ (w bg.).

In Table~\ref{table:background}, we study the impact of TW1CH in unsupervised settings when recovering complex temporal structures when varying  the ratio~($\tau$) of removing and keeping background frames. 
%\naila{more discussion needed, either here or in the method section, of tau and how it's incorporated into the modelling. More discussion on how background frames are treated}. We demonstrate this study on YTI dataset. 
We observe that, since UTE~\cite{ute_paper} trains their models on the background frames, their model overfits on the background class, as can be seen, when 99\% (i.e. $\tau=99$) of the background frames are ignored UTE performs 2.5\%/1.5\% in MoF/IoU, at the same time, when  99\% of the background frames are considered UTE performs 58.6\% in MoF -- which means that the UTE predicted majority of the frames as the background class cf. Table~\ref{table:datasets} YTI has 63.5\% background frames. Thus, we expect a drop of IoU to 2.7\%. While in case of TW1CH, when 99\% of background is considered in comparison to when ignored we see a drop of performance from 74.3 $\rightarrow$ 43.6 in MoF and 60.2 $\rightarrow$ 27.7 in IoU as expected. One can observe that TW1CH outperforms UTE by a significant margin.

\textbf{Qualitative Results.} In Fig.~\ref{fig:qual_idt} we show qualitative segmentation results on YTI dataset. For this evaluation, we use IDT features as input instead of MLP trained features used in the UTE and Mallow methods. We can clearly observe that our method predicts perfect segments wrt.  the ground-truth, while UTE and Mallow clearly fails to model the right  order of actions occurring in this video with mixed actions. \saquib{we should also discuss here about IDT features vs ute and mallow trained features etc}


\paragraph{50Salads~(FS):}\emph{ }

\textbf{Dataset.} The dataset contains an average of 19 actions per video, and 14.1\% of background frames of all frames in the whole dataset.  
% 19  14.1\%

\textbf{Results.} In Table~\ref{table:eval_fs}, we show the results. TW1CH obtains an IoU of 47.7.1\% and MoF of 66.5\%.  TW1CH is -/36.3\% and 16.2/11.8\% better than the UTE~\cite{ute_paper} and CDFL~\cite{ute_paper} in IoU/MoF metric. Also, one can observe that TW1CH is quite the matching the fully supervised performance. 
 



\paragraph{MPII Cooking 2~(MPII):}\emph{ }

\textbf{Dataset.} The dataset contains an average of 17 actions per video, and 29\% of background frames of all frames in the whole dataset.  For this dataset, we report the standard metric midpoint hit criterion~\cite{rohrbach2012database} (precision and recall), in addition to IoU and MoF.
%17 29\%

\textbf{Results.} In Table~\ref{table:eval_mpii}, we show the results. TW1CH under-performs to the state-of-the-art weakly-supervised and fully-supervised approaches, but still outperforming the baseline clustering methods by a significant margin. 


\paragraph{Hollywood Extended~(HE):}\emph{ }

\textbf{Dataset.} The dataset contains an average of 3 actions per video, and 61\% of background frames of all frames in the whole dataset.  
% 3 61\%

\textbf{Results.} In Table~\ref{table:eval_he}, we show the results.

TW1CH outperforms CDFL~\cite{cdfl}  by 19\% (38.5$\rightarrow$19.5) and 12.8\% (57.8$\rightarrow$-45) in IoU and MoF, respectively. Further, note that, baseline clustering performance is quite  matching the performance of our method, this is due to fact that there are only an average of 3 actions per video, thus FINCH is as effective as our TW1CH based temporal ordering, due to of being an easy dataset. 




\subsection{Computational complexity} As we need to compute the $N \times N$ temporal distances, the computational complexity of TW1CH is $\mathcal{O}(N^2)$. In contrast FINCH is $\mathcal{O}(Nlog(N))$.
Other similar graph-based clustering methods such as spectral methods are $\mathcal{O}(N^3)$ and hierarchical agglomerative linkage-based schemes are $\mathcal{O}(N^2log(N))$.
In Table~\ref{table:time}, we provide the total run-time of TW1CH and other state-of-the-art methods on Breakfast dataset split 1 (252 videos). Unlike previous methods that requires hours of model training on GPUs, our method essentially runs on a computer with an AMD Ryzen Threadripper 1950X 16-core processor taking approximately an average duration of $0.16$ seconds for segmenting one video ($\approx2000$ frames) in the Breakfast dataset.
%The most important benefit of our approach compared to previous method is our method requires no training. 

\begin{table}[t!]
%\footnotesize
\centering
\resizebox{8.3cm}{!}{
\begin{tabular}{ll|cc|ccc}
\toprule
	     &  \multicolumn{3}{c}{\color{blue}{Breakfast dataset}}   \\
\midrule
Supervision  &Method&IoU & MoF & A & V & T	  \\
\midrule
%ResNet-50 &\\ 
\multirow{4}{*}{\color{blue}{Fully Sup.}} 
&HOGHOF+HTK~\cite{ute_15}         &\textemdash&28.8\\
&TCFPN~\cite{ute_7}              &\textemdash&52.0\\
&HTK+DTF w. PCA~\cite{ute_16}     & 9.8 &56.3\\
&RNN+HMM~\cite{kuehne2018hybrid}            &\textemdash&61.3\\
\midrule
\multirow{8}{*}{\color{blue}{Weakly Sup.}}
&ECTC~\cite{ute_12}       &\textemdash &27.7\\
&GMM+CNN~\cite{ute_17}    &\textemdash&28.2\\
&SCT~\cite{sct}   & \textemdash &30.4  \\
&RNN-FC~\cite{ute_24} &\textemdash&33.3\\
&RNN+HMM~\cite{kuehne2018hybrid}            &\textemdash&36.7\\
&TCFPN~\cite{ute_7}      &24.2 &38.4\\
&NN-Vit.~\cite{nnv}    &\textemdash&43.0\\
&D3TW~\cite{d3tw}   &\textemdash& 45.7  \\
&MuCon~\cite{mucon} &\textemdash& 47.1 \\
&CDFL~\cite{cdfl}   &33.7& 50.2  \\
\midrule
\multirow{3}{*}{\color{blue}{Unsup. Baselines}}
& {\color{red}{Equal Split}} 
& {\color{red}{21.9}} & {\color{red}{34.8}} & \ding{51}& \ding{55}& \ding{55}\\
& Kmeans & 23.5 & 42.7 & \ding{51}& \ding{55}& \ding{55}\\
%& HAC & 28.2 & 47.2 \\
& FINCH & 28.3 & 51.9 & \ding{51}& \ding{55}& \ding{55}\\
\midrule
\multirow{4}{*}{\color{blue}{Unsup.}}
&Mallow~\cite{mallow}  & \textemdash & 34.6 & \ding{51}& \ding{51} & \ding{51}\\
&UTE~\cite{ute_paper} &\textemdash &41.8 & \ding{51}& \ding{51} & \ding{51}\\ % 26.4
&UTE~\cite{ute_paper} &\textemdash &18.3 & \ding{51}& \ding{55} & \ding{51}\\
&\textbf{Ours} & 44.1 & 63.8  & \ding{51}& \ding{55} & \ding{55}\\
%\midrule
%\multirow{1}{*}{\color{blue}{Fully Unsup.}}
%&\textbf{Ours} & 43.1 & 52.9 & \ding{55}& \ding{55} & \ding{55}\\
\bottomrule
\end{tabular}}
% \vspace{0.2cm}
\caption{Comparison of proposed method to other state-of-the-art approaches for fully, weakly and unsupervised learning on the Breakfast dataset~\cite{ute_15}. Where \textbf{A} denotes number of action classes known, \textbf{V} denotes the video activity Label known, and  \textbf{T} denotes to requires Training. The dash means no results reported by
prior work. \label{table:eval_bf}}
\end{table}


\begin{table*}[t!]
%\footnotesize
\centering

\resizebox{16.6cm}{!}{
\begin{tabular}{l|cc|cc||cc|cc}
\toprule
%\multicolumn{3}{c}{Influence of background ratio $\tau$} \\
%\midrule
	       \multicolumn{9}{c}{\color{blue}{Inria Instructional Videos}}\\
\midrule
	        &\multicolumn{4}{c}{MoF}  & \multicolumn{4}{c}{IoU}	  \\
\midrule
$\tau$ & wo bg.~\cite{ute_paper} & wo bg.~(\textbf{Ours}) &  w bg.~\cite{ute_paper}  &  w bg.~(\textbf{Ours}) & wo bg.~\cite{ute_paper} & wo bg.~(\textbf{Ours}) &  w bg.~\cite{ute_paper}  &  w bg.~(\textbf{Ours}) \\
\midrule
60 & 19.8 & 52.3  &8.0& 48.7  & 4.9 & 35.6 & 4.9 & 32.3 \\
70 & 19.6 & 56.6  &9.0& 47.9  & 4.9 & 40.0 & 4.8 & 31.7 \\
75 & 19.4 & 58.6  &10.1& 46.5 & 4.8 & 41.9 & 4.8 & 30.8 \\
80 & 18.9 & 60.3  &12.0& 45.7 & 4.8 & 43.4 & 4.9 & 29.5 \\
90 & 15.6 & 64.9  &22.7& 44.7 & 4.3 & 48.6 & 4.7 & 28.6 \\
99 & 2.5  & 74.3  &\textbf{58.6}& 43.6 & 1.5 &  60.2& 2.7 & 27.7 \\
100 & \textemdash & 79.5  & \textemdash & 43.4  & \textemdash & 69.0 & \textemdash & 27.6 \\
\bottomrule
\end{tabular}}
% \vspace{0.2cm}
\caption{ Evaluation of $\tau$ reported as MoF without~(wo bg.) and with~(w bg.) background on the YouTube Instructions dataset~\cite{yti_paper}.\label{table:background}}
\end{table*}


\begin{table}[t!]
%\footnotesize
\centering
\resizebox{8.3cm}{!}{
\begin{tabular}{ll|cc|ccc}
\toprule
	     &  \multicolumn{3}{c}{\color{blue}{Inria Instructional Videos}}   \\
\midrule
Supervision  &Method&F1-Score & MoF & A& V & T	  \\
\midrule
\multirow{3}{*}{\color{blue}{Unsup. Baselines}}
& {\color{red}{Equal Split}} 
& {\color{red}{27.8}} & {\color{red}{30.2}} & \ding{51}& \ding{55}& \ding{55}\\
& Kmeans & 29.4 & 38.5 & \ding{51}& \ding{55}& \ding{55}\\
%& HAC & 35.3 & 42.3 \\
& FINCH & 35.4 & 44.8 & \ding{51}& \ding{55}& \ding{55}\\
\midrule
\multirow{5}{*}{\color{blue}{Unsup.}}
&Frank-Wolfe~\cite{yti_paper}  &24.4 &  \textemdash& \ding{55}& \ding{51} & \ding{51}\\
&Mallow~\cite{mallow}  &27.0 &27.8 & \ding{51}& \ding{51} & \ding{51} \\
&UTE~\cite{ute_paper} &28.3 &39.0 & \ding{51} & \ding{51} & \ding{51} \\
&UTE~\cite{ute_paper} &\textemdash &19.4 & \ding{51}& \ding{55} & \ding{51}\\
&\textbf{Ours} & 51.9 & 58.6 & \ding{51}& \ding{55} & \ding{55}\\
%\midrule
%\multirow{1}{*}{\color{blue}{Fully Unsup.}}
%&\textbf{Ours} & 36.4 & 51.7 & \ding{55}& \ding{55} & \ding{55}\\
\bottomrule
\end{tabular}}
% \vspace{0.2cm}
\caption{Comparison of proposed method to other state-of-the-art unsupervised learning approaches on the Inria Instructional Videos~\cite{yti_paper}. Results are reported without background at background ratio $\tau=75\%$ as in~\cite{ute_15}. \textbf{A:} Video Activity Label known. \textbf{A:} number of action classes known. \textbf{T:} Requires Training \label{table:eval_yti}}
\end{table}



\begin{table}[t!]
%\footnotesize
\centering
\resizebox{8.3cm}{!}{
\begin{tabular}{ll|cc|ccc}
\toprule
	     &  \multicolumn{3}{c}{\color{blue}{50Salads}}   \\
\midrule
Supervision  &Method&IoU & MoF & A & V & T	  \\
\midrule
%{\color{blue}{Fully Sup.}} & \cite{ute_8} &eval &88.5\\
%\multirow{2}{*}{\color{blue}{Unsup.}}&
%\cite{ute} &eval &35.5\\
%&\textbf{Ours} & & \\
%\midrule
{\color{blue}{Fully Sup.}} & TricorNet~\cite{ute_6} &\textemdash &67.5\\
\midrule
\multirow{5}{*}{\color{blue}{Weakly Sup.}}
& ECTC~\cite{ute_12}    & \textemdash & 11.9\\
& HTK+DTF~\cite{ute_16} & \textemdash &24.7\\
& RNN-FC~\cite{ute_24}  & \textemdash &45.5\\
& NN-Vit.~\cite{nnv}    & \textemdash &49.4\\
& CDFL~\cite{cdfl}      & 31.5 &54.7\\
\midrule
\multirow{3}{*}{\color{blue}{Unsup. Baselines}}
& {\color{red}{Equal Split}} 
& {\color{red}{23.5}} & {\color{red}{33.1}}  & \ding{51}& \ding{55}& \ding{55}\\
& Kmeans & 15.7 & 29.4  & \ding{51}& \ding{55}& \ding{55}\\
%& HAC & 20.4 & 34.8 \\
& FINCH & 17.4 & 33.7 & \ding{51}& \ding{55}& \ding{55}\\
\midrule
\multirow{2}{*}{\color{blue}{Unsup.}}
& UTE~\cite{ute_paper}        & \textemdash &30.2\\
&\textbf{Ours} & 47.7 & 66.5 & \ding{51}& \ding{55} & \ding{55}\\
%\midrule
%\multirow{1}{*}{\color{blue}{Fully Unsup.}}
%&\textbf{Ours} & 42.7 & 61.9  & \ding{55}& \ding{55} & \ding{55}\\
\bottomrule
\end{tabular}}
% \vspace{0.2cm}
\caption{Comparison of proposed method to other state-of-the-art approaches for fully, weakly and unsupervised learning on the 50Salads dataset~\cite{fs_paper}. \textbf{A:} Video Activity Label known. \textbf{A:} number of sub action classes known. \textbf{T:} Requires Training \label{table:eval_fs}}
\end{table}


\begin{table}[t!]
%\footnotesize
\centering
\resizebox{8.3cm}{!}{
\begin{tabular}{ll|cccc|cccc}
\toprule
	     &  \multicolumn{5}{c}{\color{blue}{MPI Cooking 2}}   \\
\midrule
Supervision  &Method&IoU &\multicolumn{2}{c}{{Midpoint-hit}}&MoF	&A &V &T  \\
	        && &Precision &Recall&	& & &  \\
\midrule
\multirow{1}{*}{\color{blue}{Fully Sup.}}
%& Kitchen~\cite{kuehne2015cooking} &  &-& \textemdash& 57.3\\
& GMM+CNN~\cite{ute_17} & 45.5 &\textemdash& \textemdash& 72.0\\
\midrule
\multirow{1}{*}{\color{blue}{Weakly Sup.}}
%& ActionSet-MC~\cite{actionset} & \textemdash&&9.8& \textemdash\\
%& ActionSet-Text~\cite{actionset}  & \textemdash&10.6&& \textemdash \\
%& SCT~\cite{sct}                         & \textemdash&14.3 && \textemdash\\
& GMM+CNN~\cite{ute_17} & 29.7 &\textemdash& \textemdash& 59.7\\
%& Fine grained~\cite{ni2014multiple} & \textemdash  &54.3& \textemdash& \textemdash\\
\midrule
\multirow{3}{*}{\color{blue}{Unsup. Baselines}}
& {\color{red}{Equal Split}} - Testset 
& {\color{red}{6.9}} &{\color{red}{25.6}}& {\color{red}{44.6}} & {\color{red}{14.6}} & \ding{51}& \ding{55}& \ding{55} \\
& Kmeans - Testset & 14.5 &21.9& 34.8 & 30.4& \ding{51}& \ding{55}& \ding{55} \\
%& HAC - Testset &  & & \\
& FINCH - Testset & 18.3 &26.3& 41.9 &  40.5 & \ding{51}& \ding{55}& \ding{55}\\
\midrule
\multirow{1}{*}{\color{blue}{UnSup.}}
&\textbf{Ours on Test set} & 24.6 &37.5& 59.2 & 43.4 & \ding{51}& \ding{55}& \ding{55}  \\
%\midrule
%\multirow{3}{*}{\color{blue}{Baselines}}
%& Kmeans - Full & 14.0 && 21.2 & 29.9  \\
%& HAC - Full &  18.6& 19.59& 36.54\\
%& FINCH - Full & 18.2 && 23.1 & 42.1\\
%\midrule
%\multirow{1}{*}{\color{blue}{UnSup.}}
%&\textbf{Ours on Full set} & 25.5 && 18.9 & 45.2  & \ding{51}& \ding{55}& \ding{55}  \\
%\midrule
%\multirow{2}{*}{\color{blue}{Fully UnSup.}}
%&\textbf{Ours on Test set} & 15.9 & 15.1 & 38.3 & \ding{55}& \ding{55}& \ding{55}  \\
%&\textbf{Ours on Full set} & 21.3 & 14.8 & 39.4 & \ding{55}& \ding{55}& \ding{55}  \\
\bottomrule
\end{tabular}}
% \vspace{0.2cm}
\caption{Comparison of proposed method to other state-of-the-art approaches for fully, weakly and unsupervised learning on the MPII Cooking 2 dataset~\cite{mpii_paper}.\label{table:eval_mpii}}
\end{table}


\begin{table}[t!]
%\footnotesize
\centering
\resizebox{8.3cm}{!}{
\begin{tabular}{ll|cc|cccc}
\toprule
	     &  \multicolumn{5}{c}{\color{blue}{Hollywood Extended}}   \\
\midrule
Supervision  &Method&IoU & MoF &A &V &T	  \\
\midrule
\multirow{8}{*}{\color{blue}{Weakly Sup.}}
& HTK+DTF~\cite{ute_16}   & 8.6 & 33.0 &\\
& ActionSet-monte-carlo~\cite{actionset}&9.3  &\textemdash& \\
& ActionSet-text-based~\cite{actionset}  &9.2 &\textemdash& \\
& RNN-FC~\cite{ute_24}  & 11.9 &\textemdash &\\
& TCFPN~\cite{ute_7}    & 12.6 & 28.7 &\\
& SCT~\cite{sct}        & 17.7 & \textemdash& \\
& D3TW~\cite{d3tw}      & \textemdash & 33.6& \\
& CDFL~\cite{cdfl}      & 19.5 & 45.0 & \\
\midrule 
\multirow{3}{*}{\color{blue}{Unsup. Baselines}}
& {\color{red}{Equal Split}} 
& {\color{red}{24.6}} & {\color{red}{39.6}} & \ding{51}& \ding{55}& \ding{55}\\
& Kmeans & 33.2 & 55.3 & \ding{51}& \ding{55}& \ding{55}\\
%& HAC & & \\
& FINCH & 37.1 & 56.8 & \ding{51}& \ding{55}& \ding{55}\\
\midrule
\multirow{1}{*}{\color{blue}{UnSup.}}
&\textbf{Ours on full set} & 38.5  & 57.8 & \ding{51}& \ding{55}& \ding{55}  \\
%\midrule
%\multirow{1}{*}{\color{blue}{Fully UnSup.}}
%&\textbf{Ours on full set} & 36.3  & 50.1 & \ding{55}& \ding{55} & \ding{55} \\
\bottomrule
\end{tabular}}
% \vspace{0.2cm}
\caption{Comparison of proposed method to other state-of-the-art approaches for weakly and unsupervised learning on the Hollywood Extended dataset~\cite{he_paper}.\label{table:eval_he}}
\end{table}

\begin{table}[t!]
\centering
\resizebox{8.3cm}{!}{
\begin{tabular}{ll|cc|ccc}
\toprule
Supervision &Method & Training & Testing &A &V &T \\
&      & (hours) & (seconds) \\
\midrule
\multirow{4}{*}{\color{blue}{Weakly Sup.}}
&TCFPN$^{\star}$~\cite{ute_7} & 12.75 & 00.01\\
&NN-Vit.$^{\star}$~\cite{nnv} & 11.23 & 56.25\\
&CDFL$^{\star}$~\cite{cdfl}   & 66.73 & 62.37\\
&MuCon-full$^{\star}$~\cite{mucon} & 04.57 & 03.03 \\
\midrule
\multirow{2}{*}{\color{blue}{Unsup. Baselines}} 
& Kmeans & {\color{red}{00.00}} & 38.69& \ding{51}& \ding{55}& \ding{55}\\
& FINCH &  {\color{red}{00.00}} & 37.08& \ding{51}& \ding{55}& \ding{55}\\
\midrule
\multirow{2}{*}{\color{blue}{Unsupe.}} 
& UTE~\cite{ute_paper} & \textemdash & 217.94 & \ding{51}& \ding{55}& \ding{51}\\
& \textbf{Ours} & {\color{red}{00.00}} & 40.31& \ding{51}& \ding{55}& \ding{55}  \\
\bottomrule
\end{tabular} }
\vspace{0.2cm}
\caption{ Run-time comparison of method with other state-of-the-art methods for full Breakfast dataset. 
%Training and Inference Speed: Speed of training and inference for different approaches, measure as wall clock time. Training duration is measured in hours for full training on the split 1 of the Breakfast dataset.
Testing duration is measured as the average inference for split 1 test
set (252 videos).  $^{\star}$The run-time of all the {\color{blue}{Weakly Sup.}} methods were taken from~\cite{mucon}   \label{table:time}}
\end{table}
%Inference time -- UTE: 0.9047


\iffalse
\begin{table}[t!]
%\footnotesize
\centering
\caption{ Run-time comparison of method with other state-of-the-art methods for full Breakfast dataset. Training duration is measured in hours for full training on the split 1 of the Breakfast dataset.
%Training and Inference Speed: Speed of training and inference for different approaches, measure as wall clock time. Training duration is measured in hours for full training on the split 1 of the Breakfast dataset.
%Inference duration is measured as the average inference time for split 1 test set. 
 \label{table:time}}
\resizebox{8.3cm}{!}{
\begin{tabular}{l|cccc|c}
\toprule
 & TCFPN~\cite{ute_7} & NN-Vit.~\cite{nnv} &CDFL~\cite{cdfl}
&MuCon-full~\cite{mucon} &Ours \\
\midrule
T & \ding{51}& \ding{51} & \ding{51} & \ding{51} & \ding{55}  \\
\midrule
Time & 12.75 & 11.23 & 66.73 & 04.57 & {\color{red}{00.00}}\\
\bottomrule
\end{tabular}}
\end{table}
\fi

\iffalse
\begin{table*}[t!]
%\footnotesize
\centering
\caption{Comparison of our method with UTE~\cite{ute_paper} based on their Viterbi decoding.\label{table:eval_w_ute}}
\resizebox{16.6cm}{!}{
\begin{tabular}{l|lc|ccccccc|c}
\toprule
Dataset & Method & Granularity Level & MoF & MoF\_bg & IoU & IoU\_bg & P & R & F1-Score& T \\
\midrule
%BF\_Kmeans\_MoF &&& 42.34 & 42.34 & 21.63 & 21.63 & 25.53 & 37.01 & 29.20 \\
%BF\_FINCH\_MoF &&& 62.24 & 62.24 & 41.48 & 41.48 & 38.10 & 55.02 & 43.75 \\
BF & UTE~\cite{ute_paper} && 48.65 & 48.65 & 11.34 & 11.34 & 16.88 & 23.89 & 19.00 & \ding{55}\\
BF & Ours && 61.02 & 61.02 & 39.14 & 39.14 & 36.26 & 52.53 & 41.65 & \ding{55}\\
\midrule
%YTI\_Kmeans\_MoF &&& 29.05 & 41.81 & 10.70 & 16.63 & 16.57 & 23.70 & 18.86 \\
%YTI\_FINCH\_MoF &&& 35.40 & 44.24 & 17.25 & 23.20 & 22.60 & 32.49 & 25.93 \\
YTI & UTE~\cite{ute_paper}  && 33.27 & 17.62 & 3.42 & 4.74 & 11.43 & 16.20 & 12.85 & \ding{55}\\
YTI & Ours  && 69.21 & 26.74 & 26.03 & 26.38 & 44.70 & 63.79 & 51.20 & \ding{55}\\
\midrule
%FS\_Kmeans\_eval\_MoF &&& 33.32 & 33.32 & 11.71 & 11.71 & 38.98 & 26.54 & 31.34 \\
%FS\_FINCH\_eval\_MoF &&& 50.26 & 50.26 & 40.59 & 40.59 & 64.47 & 44.10 & 51.99 \\
%FS\_Kmeans\_high\_MoF &&& 43.80 & 43.80 & 15.22 & 15.22 & 26.23 & 30.07 & 27.82 \\
%FS\_FINCH\_high\_MoF &&& 43.78 & 43.78 & 53.92 & 53.92 & 48.31 & 55.95 & 51.51 \\
FS & UTE~\cite{ute_paper} & eval & 35.07 & 35.07 & 3.06 & 3.06 & 32.00 & 21.08 & 25.26 & \ding{55}\\
FS & Ours & eval & 38.83 & 38.83 & 14.73 & 14.73 & 40.13 & 26.97 & 32.02 & \ding{55}\\
FS & UTE~\cite{ute_paper} & mid & 59.09 & 59.09 & 12.33 & 12.33 & 24.83 & 27.80 & 26.01 & \ding{55}\\
FS & Ours & mid & 61.92 & 61.92 & 25.46 & 25.46 & 37.40 & 42.47 & 39.45 & \ding{55}\\
\bottomrule
\end{tabular}}
\end{table*}
\fi

\begin{figure*}
    \centering
    %\includegraphics[width=1\linewidth]{tex_files/figs/p08.png}
    %\includegraphics[width=1.08\linewidth]{tex_files/figs/p08_55.png}
    %\includegraphics[width=0.99\linewidth]{tex_files/figs/c.pdf}
    %\includegraphics[width=1\linewidth]{tex_files/figs/p03_global_local.png}
    %\includegraphics[width=1\linewidth]{tex_files/figs/p03_global_IDT.png}
    %\includegraphics[width=1\linewidth]{tex_files/figs/p23_IDT_IDT.png}
    %\includegraphics[width=1\linewidth]{tex_files/figs/p23_global_IDT.png}
    \includegraphics[width=0.485\linewidth]{tex_files/figs/P39.pdf} \quad
    \includegraphics[width=0.485\linewidth]{tex_files/figs/P46.pdf}
    % \vspace{0.2cm}
    \caption{Segmentation output examples from Breakfast Dataset~\cite{ute_15}: \textit{P39\_cam02\_P39\_scrambledegg} (\textit{left}) and \textit{P46\_webcam02\_P46\_milk}~(\textit{right}). Comparing the segmentation quality of our method to Kmeans, FINCH, and state-of-the-art unsupervised methods: UTE and Mallow. Our method has predicted the right order of actions occurring in this video with an accurate action length.  Colors indicate different actions and listed in chronological order where the predictions are color mapped one-to-one according to the ground-truth~(GT).}
    \label{fig:qual_ac}
\end{figure*}






\begin{figure}
    \centering
    %\includegraphics[width=1\linewidth]{tex_files/figs/p23_IDT_IDT.png}
    \includegraphics[width=1\linewidth]{tex_files/figs/b.pdf}
    %\includegraphics[width=1\linewidth]{tex_files/figs/p23_global_IDT.png}
    % \vspace{0.2cm}
    \caption{Segmentation output examples from  Inria  Instructional Videos dataset~\cite{yti_paper}:  \textit{changing\_tire\_0023}). Comparing the segmentation quality of our method to the unsupervised methods, UTE and Mallow. For this evaluation, we use IDT features as input instead of MLP trained features used in the UTE and Mallow methods. We can clearly observe that our method predicts perfect segments wrt. the ground-truth, while UTE and Mallow clearly fails to model the right order of actions occurring in this video with mixed actions.}
    \label{fig:qual_idt}
\end{figure}


\iffalse
\begin{table}[t!]
%\footnotesize
\centering
\caption{Purity and accuracy of automatically estimated number of sub-activities in the video for each dataset .\label{table:purity}}
%\resizebox{16.6cm}{!}{
\begin{tabular}{l|cc}
\toprule
Dataset & Purity & Accuracy \\
\midrule
BF     &  82.1    & 61.98    \\
YTI    &  81.4  & 78.5    \\
FS     &  81.5  & 90.0        \\
MPII   &  79.8  & 64.8    \\
HE     &  80.5  & 73.8    \\
\bottomrule
\end{tabular}%}
\end{table}


metrics for fuly unsupervised
 dataset                purity          K-prediction-acc-at within 1/2 gt      #avg-gt
 'BF'                    0.82086                0.61857                         6
  'YTI'                   0.81403                0.78523                        9
  'FS'                    0.81522                    0.9                        19
  'MPII_Cooking'          0.79836                0.64835                        17
  'Hollywood_extended'    0.80531                0.73853                        3

\fi
